PICE: A Semantic-Driven Progressive Inference System for LLM Serving in Cloud-Edge Networks

Large language models (LLMs), while driving a new wave of interactive AI applications across numerous domains, suffer from high inference costs and heavy cloud dependency. Motivated by the redundancy phenomenon in linguistics, we propose a progressive inference paradigm over cloud and edge, i.e., firstly generating the sketch of the answer by LLMs at cloud, and then conducting parallel extension to fill in details by small models (SLMs) at edge. Progressive inference offers potential benefits to improve throughput and reduce inference latency while facing key implementation challenges, including decreased response quality from SLMs, a tradeoff between the brevity and comprehensiveness of sketches, as well as increased latency caused by network transmission and edge inference. In this work, we propose and implement PICE, an LLM serving system with semantic-level cloud-edge collaboration, enhancing inference throughput and quality through dynamic inference task scheduling, ensemble learning, and parallel edge inference. Extensive testbed experiments illustrate that our approach achieves $1.5-2\times$ throughput enhancement and up to 43% latency reduction, while also potentially enhancing the quality compared to SOTA systems.

==> chapter/biography.tex <==
% \newpage

% \section{Biography Section}
% If you have an EPS/PDF photo (graphicx package needed), extra braces are
%  needed around the contents of the optional argument to biography to prevent
%  the LaTeX parser from getting confused when it sees the complicated
%  $\backslash${\tt{includegraphics}} command within an optional argument. (You can create
%  your own custom macro containing the $\backslash${\tt{includegraphics}} command to make things
%  simpler here.)
 
% \vspace{11pt}

% \bf{If you include a photo:}\vspace{-33pt}
% \begin{IEEEbiography}
% [{\includegraphics[width=1in,height=0.8in,clip,keepaspectratio]{Huiyou Zhan}
% received her B.Eng. degree in University of Science and Technology of
% China (USTC) in 2020. She is currently pursuing her Ph.D degree at University of Science and Technology of China (USTC). Her main research interest is cloud computing, edge computing and algorithm design.
% \end{IEEEbiography}



\begin{IEEEbiography}
[{\includegraphics[width=0.9in,height=1.1in]{figure/photo/Zhan.jpg}}]{Huiyou Zhan} received her B.Eng. degree in University of Science and Technology of China (USTC) in 2020. She is currently pursuing her Ph.D degree at University of Science and Technology of China (USTC). Her main research interest is cloud computing, edge computing and Online Algorithms.
\end{IEEEbiography}

\begin{IEEEbiography}
[{\includegraphics[width=0.9in,height=1.1in]{figure/photo/Zhang.jpg}}]{Xuan Zhang} received her B.Eng.  degree  in Computer Science and Technology from Northwest University, China, in 2023. She is currently pursuing her MS degree at University of Science and Technology of China (USTC). Her main research interest is edge computing and system for ai.
\end{IEEEbiography}

\begin{IEEEbiography}
[{\includegraphics[width=1in,height=1.25in]{figure/photo/Tan.jpg}}]{Haisheng Tan} (Seniro Member, IEEE) received his B.E. degree in Software Engineering and B.S. degree in Management both from University of Science and Technology of China (USTC) with the highest honor. Then, he got his Ph.D. degree in computer science at the University of Hong Kong (HKU). He is currently a professor at USTC. His research interests include algorithms and networking. Dr. Tan has published over 80 papers in prestigious journals and conferences, mainly in the areas of AIoT and edge computing. He recently received the Best Paper Award in WASA’19, CWSN’20, PDCAT’20, and ICAPDS’21.
\end{IEEEbiography}

\begin{IEEEbiography}
[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{figure/photo/tian.jpg}}]{Han Tian} is currently an assistant researcher in the University of Science and Technology of China. He received his Ph.D. in the Hong Kong University of Science and Technology, supervised by Prof. Kai Chen and Prof. Qiang Yang. He received his B.Eng from Beihang University in 2012 and M.Eng in Computer Science from Sun Yat-sen University.  Han's research interests span machine learning and its applications including networking, system and private computing. He has authored and co-authored several referred journals and proceedings including IEEE S\&P, CoNEXT, and EuroSys.
\end{IEEEbiography}

\begin{IEEEbiography}
[{\includegraphics[width=0.9in,height=1.1in]{figure/photo/Yong.jpg}}]{Dongping Yong} is currently pursuing a Ph.D. at the University of Science and Technology of China. She holds a Master's degree in Computer Science and Technology from Southwest University of Science and Technology. Her research interests encompass task scheduling and edge AI.
\end{IEEEbiography}



\begin{IEEEbiography}
[{\includegraphics[width=0.9in,height=1.15in]{figure/photo/ZhangJY.jpg}}]{Junyang Zhang}
is a Ph.D. candidate at the School of Computer Science and Technology, University of Science and Technology of China (USTC). His research interests focus on intelligent sensing and model inference.
\end{IEEEbiography}


\begin{IEEEbiography}
[{\includegraphics[width=0.95in,height=1.25in]{figure/photo/Li.png}}]{Xiang-Yang Li} (Fellow, IEEE/ACM) is a full professor and executive dean at School of Computer Science and Technology, USTC, Hefei, China. He was a full professor at Illinois Institute of Technology, Chicago, USA. He is an ACM/IEEE Fellow and an ACM Distinguished Scientist. Dr. Li received MS (2000) and PhD (2001) degree at Department of Computer Science from University of Illinois at Urbana-Champaign, a Bachelor degree at Department of Computer Science and a Bachelor degree at Department of Business Management from Tsinghua University, both in 1995. His research span Artificial Intelligent Internet of Things, mobile computing, data sharing and trading, and privacy. He published a monograph “Wireless Ad Hoc and Sensor Networks: Theory and Applications”.
\end{IEEEbiography}

% \vspace{11pt}

% \bf{If you will not include a photo:}\vspace{-33pt}
% \begin{IEEEbiographynophoto}{John Doe}
% Use $\backslash${\tt{begin\{IEEEbiographynophoto\}}} and the author name as the argument followed by the biography text.
% \end{IEEEbiographynophoto}

==> chapter/test.tex <==

\section{Introduction}
Large-scale language models (LLMs) such as GPT4, LLaMA, and Qwen \cite{achiam2023gpt, touvron2023llama, bai2023qwen} have exhibited unprecedented performance in natural language processing and chatbot systems. However, the exceptional capabilities of LLMs come at a significant inference cost, taking 22 seconds for Claude \cite{claude} (accessed through Slack API) and 43 seconds for Vicuna-33B \cite{chiang2023vicuna} (running locally on one NVIDIA A100 GPU) to generate a response \cite{ning2024skeleton}. 
To efficiently serve LLMs has emerged as a crucial demand for LLM-based AI applications to provide an engaging user experience, as their interactive nature mandates low response latency and high throughput during inference.


Moreover, due to the massive size of LLMs, current systems heavily rely on cloud computing  (Fig. \ref{fig:example}(a) - left), suffering from heavy request loads, high operational costs, and privacy concerns~\cite{zhang2024edgeshard}. To mitigate these issues, there has been a growing interest in designing smaller, cost-effective LLMs that can take advantage of the increasing availability of numerous and diverse edge computing devices. For instance, Meta provides multiple versions of Llama \cite{touvron2023llama} with only 7 billion parameters small enough to run on edge devices (Fig. \ref{fig:example}(a) - middle). Although this approach can enhance efficiency, it typically compromises response quality. To balance the need for fast and cost-effective inference, a hybrid inference strategy has been proposed, utilizing a router to dynamically allocate queries to either a small model on the edge or a large model on the cloud based on the predicted query difficulty \cite{ding2024hybrid, ong2024routellm, zhang2024treacle} (Fig. \ref{fig:example}(a) - right). However, this coarse-grained scheduling method is overly reliant on the performance of the router, highlighting the need for a more generalized approach that effectively harmonizes inference efficiency with response quality.


\begin{figure}[htbp]
    \centering
    \includegraphics[width=0.98\columnwidth]{figure/not_lab/example.pdf}
    \caption{Existing inference paradigms vs. progressive inference.} 
    \label{fig:example}
\end{figure}


In contrast to existing efforts on optimizing inference at the model and system levels, we take a ``semantic-level” pathway to improve throughput by reducing the output of LLMs, \ie, \emph{the LLM creates the response sketch and the SLM fills in the details}. This perspective stems from how humans answer questions, \ie, we can convey the general meaning of a sentence with just a few words. 


Motivated by this idea, we propose a progressive inference paradigm over cloud and edge (Fig. \ref{fig:example}(b)). This architecture leverages the redundant computing power on the edge to offload workloads from the cloud while ensuring high response quality. Specifically, upon receiving a query, the LLM first evaluates the potential length of the response. If the response is concise and short, LLM will directly output a complete answer. In cases where a lengthy response is anticipated, LLM will produce semantically complete yet minimally grammatical sketches and then SLMs on the edge perform extension to improve inference efficiency. The semantic completeness of each short sentence eliminates sequential dependencies for their expansions, enabling SLMs to process each sentence in parallel and thereby breaking the sequential decoding of autoregressive models.

The progressive inference paradigm is promising while introducing several key challenges in practical implementation: 1) The quality of responses from SLMs may decline; 2) The tradeoff between the brevity and the quality of LLM's sketches, \ie, while shorter sketches can improve throughput, the semantics expressed may be incomplete; and 3) Additional latency caused by network transmission and edge inference. 

In this work, we present \ouralg, an efficient progressive inference system of LLMs, which synergistically makes use of the resources at the cloud and edge, effectively reducing the workload of LLMs on the cloud, and achieving both high throughput and superior response quality. The effectiveness of \ouralg~stems from four critical designs: a specialized fine-tuning component that enables LLMs to generate concise yet semantically complete sketches, a dynamic scheduler taking advantage of progressive inference to optimize throughput, an ensemble learning mechanism aggregating outputs from multiple small models to improve quality, and a parallel execution optimization strategy for SLMs to speed up edge inference. Our main contributions are highlighted as follows.

\begin{itemize}[leftmargin=*]
    \item We propose and demonstrate the feasibility of synergistic progressive inference at the semantic-level parallel data processing across the cloud and edge. To the best of our knowledge, this is the first attempt to involve semantic optimization with cloud-edge collaboration to enable efficient and reliable LLM serving (Sec. \ref{sec:motivation}).
    \item We design \ouralg, a novel \underline{P}rogressive \underline{I}nference engine for LLM serving over \underline{C}loud and \underline{E}dge, achieving high throughput and low latency by employing model fine-tuning, dynamic scheduling, ensemble learning and parallel edge inference (Sec. \ref{sec:overview} and Sec. \ref{sec:design}). 
    \item By implementing  \ouralg~at a testbed with a set of Jetson AGX Orins and a cloud server, we conduct extensive experiments across various LLM benchmarks and popular language models, demonstrating that \ouralg~achieves a throughput enhancement of 1.5$\times$ to 2$\times$ and a latency reduction by up to 43\%, while potentially enhancing the answer quality on several question categories compared to baselines (Sec. \ref{sec:evaluation}). 
\end{itemize}

